The Host Galaxies of Rapidly Evolving Transients in the Dark Energy Survey

Rapidly evolving transients (RETs), also termed fast blue optical transients (FBOTs), are a distinct class of astrophysical event. They are characterised by lightcurves that decline much faster than common classes supernovae (SNe), span vast ranges in peak luminosity and can be seen to redshifts greater than 1. Their evolution on fast timescales has hindered high quality follow-up observations, and thus their origin and explosion/emission mechanism remains unexplained. In this paper we define the largest sample of RETs to date, comprising 106 objects from the Dark Energy Survey, and perform the most comprehensive analysis of RET host galaxies. Using deep-stacked photometry and emission-lines from OzDES spectroscopy, we derive stellar masses and star-formation rates (SFRs) for 49 host galaxies, and metallicities for 37. We find that RETs explode exclusively in star-forming galaxies and are thus likely associated with massive stars. Comparing RET hosts to samples of host galaxies of other explosive transients as well as field galaxies, we find that RETs prefer galaxies with high specific SFRs, indicating a link to young stellar populations, similar to stripped-envelope SNe. RET hosts appear to show a lack of chemical enrichment, their metallicities akin to long duration gamma-ray bursts and superluminous SN host galaxies. There are no clear relationships between properties of the host galaxies and the peak magnitudes or decline rates of the transients themselves.

==> author_list_07_May.tex <==
% Author list file generated with: mkauthlist.py 0+unknown 
% mkauthlist.py -f -a order.csv -j mnras -sb author_list_07_May.csv author_list_07_May.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
P.~Wiseman,$^{1}$
M.~Pursiainen,$^{1}$
M.~Childress,$^{1}$
E.~Swann,$^{2}$
M.~Smith,$^{1}$
L.~Galbany,$^{3}$
C.~Lidman,$^{4}$
T.~M.~Davis,$^{5}$
C.~P.~Guti\'errez,$^{1}$
A.~M\"oller,$^{6}$
B.~P.~Thomas,$^{2}$
C.~Frohmaier,$^{2}$
R.~J.~Foley,$^{7}$
S.~R.~Hinton,$^{5}$
L.~Kelsey,$^{1}$
R.~Kessler,$^{8,9}$
G.~F.~Lewis,$^{10}$
M.~Sako,$^{11}$
D.~Scolnic,$^{12}$
M.~Sullivan,$^{1}$
M.~Vincenzi,$^{2}$
T.~M.~C.~Abbott,$^{13}$
M.~Aguena,$^{14,15}$
S.~Allam,$^{16}$
J.~Annis,$^{16}$
E.~Bertin,$^{17,18}$
S.~Bhargava,$^{19}$
D.~Brooks,$^{20}$
D.~L.~Burke,$^{21,22}$
A.~Carnero~Rosell,$^{23}$
D.~Carollo,$^{24}$
M.~Carrasco~Kind,$^{25,26}$
J.~Carretero,$^{27}$
M.~Costanzi,$^{28,29}$
L.~N.~da Costa,$^{15,30}$
H.~T.~Diehl,$^{16}$
P.~Doel,$^{20}$
S.~Everett,$^{7}$
J.~Frieman,$^{16,9}$
J.~Garc\'ia-Bellido,$^{31}$
E.~Gaztanaga,$^{32,33}$
K.~Glazebrook,$^{34}$
D.~Gruen,$^{35,21,22}$
R.~A.~Gruendl,$^{25,26}$
J.~Gschwend,$^{15,30}$
G.~Gutierrez,$^{16}$
K.~Honscheid,$^{36,37}$
D.~J.~James,$^{38}$
K.~Kuehn,$^{39,40}$
N.~Kuropatkin,$^{16}$
M.~Lima,$^{14,15}$
M.~A.~G.~Maia,$^{15,30}$
J.~L.~Marshall,$^{41}$
P.~Martini,$^{36,42}$
F.~Menanteau,$^{25,26}$
R.~Miquel,$^{43,27}$
A.~Palmese,$^{16,9}$
F.~Paz-Chinch\'{o}n,$^{44,26}$
A.~A.~Plazas,$^{45}$
A.~K.~Romer,$^{19}$
E.~Sanchez,$^{23}$
M.~Schubnell,$^{46}$
S.~Serrano,$^{32,33}$
I.~Sevilla-Noarbe,$^{23}$
N.~E.~Sommer,$^{4}$
E.~Suchyta,$^{47}$
M.~E.~C.~Swanson,$^{26}$
G.~Tarle,$^{46}$
B.~E.~Tucker,$^{4}$
D.~L.~Tucker,$^{16}$
T.~N.~Varga,$^{48,49}$
and A.~R.~Walker$^{13}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{2}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{3}$ PITT PACC, Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh, PA 15260, USA\\
$^{4}$ The Research School of Astronomy and Astrophysics, Australian National University, ACT 2601, Australia\\
$^{5}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{6}$ Universit\'e Clermont Auvergne, CNRS/IN2P3, LPC, F-63000 Clermont-Ferrand, France\\
$^{7}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{8}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{9}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{10}$ Sydney Institute for Astronomy, School of Physics, A28, The University of Sydney, NSW 2006, Australia\\
$^{11}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{12}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{13}$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile\\
$^{14}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{15}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{16}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{17}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{18}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{19}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{20}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{21}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{22}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{23}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{24}$ INAF, Astrophysical Observatory of Turin, I-10025 Pino Torinese, Italy\\
$^{25}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{26}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{27}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{28}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{29}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{30}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{31}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{32}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{33}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{34}$ Centre for Astrophysics \& Supercomputing, Swinburne University of Technology, Victoria 3122, Australia\\
$^{35}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{36}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{37}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{38}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{39}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{40}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{41}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{42}$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA\\
$^{43}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{44}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{45}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{46}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{47}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{48}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{49}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
}
}


==> author_list_16_May.tex <==
% Author list file generated with: mkauthlist.py 0+unknown 
% mkauthlist.py -f -a DES-RET-Hosts/order.csv -s -j mnras DES-RET-Hosts/author_list_16_May.csv DES-RET-Hosts/author_list_16_May.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
P.~Wiseman,$^{1}$
M.~Pursiainen,$^{1}$
M.~Childress,$^{1}$
E.~Swann,$^{2}$
M.~Smith,$^{1}$
L.~Galbany,$^{3}$
C.~Lidman,$^{4}$
T.~M.~Davis,$^{5}$
C.~P.~Guti\'errez,$^{1}$
A.~M\"oller,$^{6}$
B.~P.~Thomas,$^{2}$
C.~Frohmaier,$^{2}$
R.~J.~Foley,$^{7}$
S.~R.~Hinton,$^{5}$
L.~Kelsey,$^{1}$
R.~Kessler,$^{8,9}$
G.~F.~Lewis,$^{10}$
M.~Sako,$^{11}$
D.~Scolnic,$^{12}$
M.~Sullivan,$^{1}$
M.~Vincenzi,$^{2}$
T.~M.~C.~Abbott,$^{13}$
M.~Aguena,$^{14,15}$
S.~Allam,$^{16}$
J.~Annis,$^{16}$
E.~Bertin,$^{17,18}$
S.~Bhargava,$^{19}$
D.~Brooks,$^{20}$
D.~L.~Burke,$^{21,22}$
A.~Carnero~Rosell,$^{23}$
D.~Carollo,$^{24}$
M.~Carrasco~Kind,$^{25,26}$
J.~Carretero,$^{27}$
M.~Costanzi,$^{28,29}$
L.~N.~da Costa,$^{15,30}$
H.~T.~Diehl,$^{16}$
P.~Doel,$^{20}$
S.~Everett,$^{7}$
P.~Fosalba,$^{31,32}$
J.~Frieman,$^{16,9}$
J.~Garc\'ia-Bellido,$^{33}$
E.~Gaztanaga,$^{31,32}$
K.~Glazebrook,$^{34}$
D.~Gruen,$^{35,21,22}$
R.~A.~Gruendl,$^{25,26}$
J.~Gschwend,$^{15,30}$
G.~Gutierrez,$^{16}$
D.~L.~Hollowood,$^{7}$
K.~Honscheid,$^{36,37}$
D.~J.~James,$^{38}$
K.~Kuehn,$^{39,40}$
N.~Kuropatkin,$^{16}$
M.~Lima,$^{14,15}$
M.~A.~G.~Maia,$^{15,30}$
J.~L.~Marshall,$^{41}$
P.~Martini,$^{36,42}$
F.~Menanteau,$^{25,26}$
R.~Miquel,$^{43,27}$
A.~Palmese,$^{16,9}$
F.~Paz-Chinch\'{o}n,$^{44,26}$
A.~A.~Plazas,$^{45}$
A.~K.~Romer,$^{19}$
E.~Sanchez,$^{23}$
V.~Scarpine,$^{16}$
M.~Schubnell,$^{46}$
S.~Serrano,$^{31,32}$
I.~Sevilla-Noarbe,$^{23}$
N.~E.~Sommer,$^{4}$
E.~Suchyta,$^{47}$
M.~E.~C.~Swanson,$^{26}$
G.~Tarle,$^{46}$
B.~E.~Tucker,$^{4}$
D.~L.~Tucker,$^{16}$
T.~N.~Varga,$^{48,49}$
and A.~R.~Walker$^{13}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{2}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{3}$ PITT PACC, Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh, PA 15260, USA\\
$^{4}$ The Research School of Astronomy and Astrophysics, Australian National University, ACT 2601, Australia\\
$^{5}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{6}$ Universit\'e Clermont Auvergne, CNRS/IN2P3, LPC, F-63000 Clermont-Ferrand, France\\
$^{7}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{8}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{9}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{10}$ Sydney Institute for Astronomy, School of Physics, A28, The University of Sydney, NSW 2006, Australia\\
$^{11}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{12}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{13}$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile\\
$^{14}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{15}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{16}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{17}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{18}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{19}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{20}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{21}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{22}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{23}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{24}$ INAF, Astrophysical Observatory of Turin, I-10025 Pino Torinese, Italy\\
$^{25}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{26}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{27}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{28}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{29}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{30}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{31}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{32}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{33}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{34}$ Centre for Astrophysics \& Supercomputing, Swinburne University of Technology, Victoria 3122, Australia\\
$^{35}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{36}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{37}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{38}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{39}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{40}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{41}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{42}$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA\\
$^{43}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{44}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{45}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{46}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{47}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{48}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{49}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
}
}

